Dependent-Type-Preserving Memory Allocation

Dependently typed programming languages such as Coq, Agda, Idris, and F*, allow programmers to write detailed specifications of their programs and prove their programs meet these specifications. However, these specifications can be violated during compilation since they are erased after type checking. External programs linked with the compiled program can violate the specifications of the original program and change the behavior of the compiled program -- even when compiled with a verified compiler. For example, since Coq does not allow explicitly allocating memory, a programmer might link their Coq program with a C program that can allocate memory. Even if the Coq program is compiled with a verified compiler, the external C program can still violate the memory-safe specification of the Coq program by providing an uninitialized pointer to memory. This error could be ruled out by type checking in a language expressive enough to indicate whether memory is initialized versus uninitialized. Linking with a program with an uninitialized pointer could be considered ill-typed, and our linking process could prevent linking with ill-typed programs. To facilitate type checking during linking, we can use type-preserving compilation, which preserves the types through the compilation process. In this ongoing work, we develop a typed intermediate language that supports dependent memory allocation, as well as a dependent-type-preserving compiler pass for memory allocation.

==> acmart-preload-hook.tex <==
\PassOptionsToPackage{dvipsnames}{xcolor}
% Fix font issue
\RequirePackage{scrlfile}
\PreventPackageFromLoading{fontenc}
\AfterPackage{newtxmath}{
  \UnPreventPackageFromLoading{fontenc}
}
% to prevent \Bbbk defined issue
\PreventPackageFromLoading{amssymb}


==> defs.tex <==
\newcommand{\len}[1]{|#1|}
\makeatletter


\newenvironment{proofcases}
%{\begin{enumerate}[label={\bfseries Case:},labelwidth=-2.8em,itemindent=0pt,leftmargin=0em]\ignorespacesafterend}%
{\begin{enumerate}[label={\bfseries Case:},labelwidth=-2em,itemindent=0pt,leftmargin=1em]\ignorespacesafterend}
{\end{enumerate}}

\newcommand{\defn}[3]{#1 \stackrel{\delta}{=} #2 : #3}

%% NB: Removes parens around argument from \@fune
\renewcommand{\@fune}[4]{%
  \kwopen{#1{\uplambda}}%
  {#2} \mathbin{:} {#3}% \mathbin{:} spacing would be a bit too large
  \mathclose{.}%
  \mathpunct{}#4}

\makeatother

%% TODO: Things that should be in mttex
\newtheorem{digression}{Digression}

%\newcommand{\im}{\inlinemath}
\newcommand{\figuretextmath}[1]{\(#1\)}
\newcommand{\figm}{\figuretextmath}
%\newcommand{\bnflabel}[1]{\mbox{\textit{#1}}}
%\newcommand{\judgshape}[2][]{\begin{flushleft}\fbox{\figm{#2}~#1}\end{flushleft}}

\newenvironment{inlinedisplay}
{\begin{displaymath}\nop}
{\end{displaymath}\nop\ignorespacesafterend}

\newenvironment{figuredisplaymath}
{\begin{displaymath}\ignorespaces}
{\end{displaymath}\nop\ignorespacesafterend}

\newcommand{\fixenumeratelemma}{~\vspace{-\baselineskip}}

% CC-CC
\renewcommand{\slang}{\text{CC-CC}\xspace}

\renewcommand{\scolor}[1]{\mathcolor{RoyalBlue}{#1}}

\newlanguage{\scolor}{\sfont}{\sfontsym}{s}
{x,y,e,t,U,i,f,A,B,v,a,n}
{lenv/\Gamma,subst/\gamma,alpha/\alpha,beta/\beta}
{npi,pi,nsigma,exist,unit,star,box,unit,pair,sigma,code,exist,nexist,trlufun}
{nfun,app,alet,dnpair,fst,snd,prj,unit,npair,let,dpair,pair,clo,utclo}

\renewcommand{\step}{\vartriangleright}
\renewcommand{\stepstar}{\step^*}

\newcommand{\subtypesym}{\preceq}
\newcommand{\sstepjudg}[4][\step]{\wf{#2}{#3\mathbin{#1}#4}}
\newcommand{\sequivjudg}[3]{\wf{#1}{#2\mathbin{\equiv}#3}}
\newcommand{\ssubtyjudg}[3]{\wf{#1}{#2\mathbin{\subtypesym}#3}}
\newcommand{\styjudg}[3]{\judg{#1}{#2}{#3}}

%\newcommand{\rulename}[1]{[{\scshape #1}]}

\newcommand{\swf}[1]{\wf{}{#1}}

\newcommand{\DFV}[2]{\metafont{FV}{(#2, #1)}}

% Linking
\newcommand{\ssubstok}[2]{\wf{#1}{#2}}

% CC-CC

\makeatletter
%% NB: Dependent versions of exists

% \@existty formats an existential type
%
% #1 : A formatting macro for symbols, such as \tfontsym
% #2 : The pre-formatted type-variable to bind
% #3 : The pre-formatted type of the type-variable.
% #4 : The pre-formatted result in which the type-variable is bound.
\renewcommand{\@existty}[4]{
  \kwopen{#1{\exists}}%
  {#2} \mathbin{:} {#3}%
  \mathclose{.}%
  \mathpunct{}#4}

% \existty is like \@existty but provides a standard interface.
%
% #1 : A formatting macro for symbols, such as \tfontsym.
% #2 : A formatting macro for text, such as \tfont.
% #3 : The pre-formatted variable the function binds.
% #4 : The pre-formatted type of the variable.
% #5 : The pre-formatted body of the function.
\renewcommand{\existty}[2]{\@existty{#1}}

% \@nexistty formats an n-ary existential type
%
% #1 : A formatting macro for symbols, such as \tfontsym
% #2 : The pre-formatted list of bindings
%\newcommand{\@nexistty}[2]{
%  \kwopen{#1{\exists}}%
%  #2%
%}

% \nexistty is like \@nexistty but provides a standard interface.
%
% #1 : A formatting macro for symbols, such as \tfontsym.
% #2 : A formatting macro for text, such as \tfont.
% #3 : The pre-formatted list of bindings.
%\newcommand{\nexistty}[2]{\@nexistty{#1}}

\newcommand{\trlufunarrow}{\Rightarrow}

% \@trlufunty formats a translucent function type.
%
% #1 : A formatting macro for symbols, such as \tfontsym
% #2 : The pre-formatted argument to the function
% #3 : The pre-formatted result of the function
\newcommand{\@trlufunty}[3]{#2 \mathbin{#1{\trlufunarrow}} #3}

% \trlufunty is like \@trlufunty but provides a interface.
%
% #1 : A formatting macro for symbols, such as \tfontsym
% #2 : A formatting macro for text, such as \tfont
% #3 : The pre-formatted argument to the function
% #4 : The pre-formatted result of the function
\newcommand{\trlufunty}[2]{\@trlufunty{#1}}

\newcommand{\codety}[4]{
  \kwopen{#2{Code}}(#3)\mathpunct{#2{.}}#4%
}

\newcommand{\cloe}[5]{
  #2{\langle\!\langle}#3\mathpunct{#2{,}}#4#2{\rangle\!\rangle}%
  \kwbin{#2{as}}%
  #5
}

\newcommand{\utcloe}[4]{
  #2{\langle\!\langle}#3\mathpunct{#2{,}}#4#2{\rangle\!\rangle}%
}

\newcommand{\ctage}[3]{
  \kwopen{#2{Clos}} #3%
}

\newcommand{\malloce}[5]{
  \kwopen{#2{malloc_{#3}}}[#4\mathpunct{#2{,}}#5]%
}

\newcommand{\assonee}[4]{
  #3[#2{1}]#2{\leftarrow} #4%
}

\newcommand{\asstwoe}[4]{
  #3[#2{2}]#2{\leftarrow} #4%
}

\newcommand{\init}[2]{
  #1^{#2}
}

\makeatother

\newcommand{\twf}[2]{\wf{#1}{#2}}
\newcommand{\tstepjudg}[5][\step]{\wf{#2\mathpunct{;}#3}{#4\mathbin{#1}#5}}
\newcommand{\tequivjudg}[4]{\wf{#1\mathpunct{;}#2}{#3\mathbin{\equiv}#4}}
\newcommand{\tsubtyjudg}[4]{\wf{#1\mathpunct{;}#2}{#3\mathbin{\subtypesym}#4}}
\newcommand{\ttyjudg}[4]{\judg{#1\mathpunct{;}#2}{#3}{#4}}

\renewcommand{\tlang}{\text{CC-CC$_A$}\xspace}

\renewcommand{\tcolor}[1]{\mathcolor{OrangeRed}{#1}}
\newlanguage{\tcolor}{\tfont}{\tfontsym}{t}
{k,x,y,e,A,B,C,U,f,v,a,n,m,t,H,h,l}
{alpha/\alpha,lenv/\Gamma,subst/\gamma,beta/\beta,phi/\phi,psi/\psi,Psi/\Psi}
{npi,pi,nsigma,exist,unit,star,box,unit,pair,sigma,code,exist,nexist,trlufun}
{nfun,app,alet,dnpair,fst,snd,prj,unit,npair,let,dpair,pair,clo,ctag,malloc,assone,asstwo}

\newcommand{\thenv}{\tPsi}
\newcommand{\thenvpr}{\tPsipr}
\newcommand{\tfl}{\tfonttext{\im{\ell}}}
\newcommand{\locmap}[2]{#1\mathbin{\mapsto}#2}

% reduction relation now with heaps, baby
\newcommand{\conf}[2]{\langle #1 \mid  #2 \rangle}

%% TODO: Add support for this pattern in mttex
\newcommand{\ttprin}[1]{\ttmetavar{#1}{}{1}}
\newcommand{\teprin}[1]{\temetavar{#1}{}{1}}

\newcommand{\all}[1]{\sembrace{#1}}


% Model Translation
\newcommand{\mlang}{CIC}
\newcommand{\model}[1]{\sembrace{#1}_{M}}

\newcommand{\mcolor}[1]{#1}
\newcommand{\mfont}[1]{#1}
\newcommand{\mfontsym}[1]{#1}
\newcommand{\mfonttext}[1]{\im{\text{#1}}}

\newlanguage{\mcolor}{\mfont}{\mfontsym}{m}
{x,y,e,U,A,B,p}
{lenv/\Gamma}
{pi,unit,star,box,sigma}
{fun,app,dpair,pair,clo,fst,snd}

\newcommand{\mnone}{\text{None}}
\newcommand{\mmaybe}[1]{\text{Maybe}~#1}
\newcommand{\mjust}[1]{\text{Just}~#1}
\newcommand{\mrefl}[1]{(\text{refl}~#1)}
\newcommand{\mmfst}[2]{(\text{maybe-fst}~#1~#2)}
\newcommand{\mmsnd}[2]{(\text{maybe-snd}~#1~#2)}


